Instructions are all you need: Self-supervised Reinforcement Learning for Instruction Following

Language models often struggle to follow multi-constraint instructions that are crucial for real-world applications. Existing reinforcement learning (RL) approaches suffer from dependency on external supervision and sparse reward signals from multi-constraint tasks. We propose a label-free self-supervised RL framework that eliminates dependency on external supervision by deriving reward signals directly from instructions and generating pseudo-labels for reward model training. Our approach introduces constraint decomposition strategies and efficient constraint-wise binary classification to address sparse reward challenges while maintaining computational efficiency. Experiments show that our approach generalizes well, achieving strong improvements across 3 in-domain and 5 out-of-domain datasets, including challenging agentic and multi-turn instruction following. The data and code are publicly available at https://github.com/Rainier-rq/verl-if

==> tables/hard.tex <==
\begin{table}[t]

\renewcommand{\arraystretch}{0.9}
\resizebox{1.0\columnwidth}{!}{
\begin{tabular}{lccccc}
\toprule
Method & Pr. (S) & Ins. (S) & Pr. (L) & Ins. (L) & Avg. \\ 
\midrule


Qwen2.5-7B-Instruct & 71.5 & 79.1 & 73.9 & 81.3 & 76.5 \\

Qwen2.5-7B-Instruct-IF & 76.7 & 83.3 & 78.9 & 85.3 & 81.1 \\

\midrule

R1-Distill-Qwen-1.5B & 38.1 & 50.4 & 42.3 & 54.3 & 46.3\\ 
R1-Distill-Qwen-1.5B-IF & 54.0 & 65.8 & 58.8 & 69.8 & 62.1 \\
R1-Distill-Qwen-7B & 56.7 & 68.3 & 61.7 & 72.5 & 64.8 \\ 
R1-Distill-Qwen-7B-IF & 65.8 & 75.2 & 71.7 & 80.2 & 73.2 \\ 
R1-0528-Qwen3-8B &74.9 & 82.4 & 79.7 & 85.9 & 80.7\\ 
R1-0528-Qwen3-8B-IF &83.5 & 88.7 & 87.1 & 91.2 & 87.6 \\
\bottomrule
\end{tabular}
}
\caption{Full results on IFEval. “Pr.” and “Ins.” refer to prompt-level and instruction-level metrics, respectively, while “S” and “L” denote strict and loose evaluation.}
   \label{tab:hard}
\end{table}
